Beyond the Interface: Redefining UX for Society-in-the-Loop AI Systems

Artificial intelligence systems increasingly operate in decision-critical environments where probabilistic outputs and Human-in-the-Loop (HITL) interactions reshape user engagement. Traditional user experience (UX) frameworks, designed for deterministic systems, fail to capture these evolving sociotechnical dynamics. This paper argues that in AI-enabled HITL systems, UX must transcend frontend usability to encompass backend performance, organizational workflows, and decision making structures. We employ a mixed-methods approach, combining an inductive social construction analysis of 269 stakeholder insights with the deployment of an operational HITL video anomaly detection system. Our findings reveal that stakeholders experience AI through multifaceted themes: risk, governance, and organizational capacity. Experimental results further demonstrate how detection behavior and alert routing directly calibrate human oversight and workload. Grounded in these results, we formalize a new evaluative framework centered on four sociotechnical metrics: Accuracy (FPR/FNR), Operational Latency (response time), Adaptation Time (deployment burden), and Trust (validated automation scales). This framework redefines UX as a multi-layered construct spanning infrastructure and governance, providing a rigorous foundation for evaluating AI systems embedded within complex real-world ecosystems.

==> Table_2.tex <==
\subsection{Interview-Derived Metrics}

The following table summarizes the metrics identified through qualitative coding of 114 semi-structured interviews.
Frequencies represent the number of interviews in which each metric was mentioned at least once.
Each interview was treated as a single unit of analysis (N = 114).
\begin{table}[h!]
\centering
\caption{Interview-Derived Metrics and Mention Frequency (N = 114)}
\label{tab:metric_frequency}
\begin{tabular}{|l|l|c|}
\hline
\textbf{Metric Category} & \textbf{Metric} & \textbf{Interviews Mentioned (N=114)} \\
\hline
Temporal & Number of People per Hour & XX \\
Temporal & Dwell Time & XX \\
Temporal & Peak Usage Prediction & XX \\
Temporal & Entry/Exit Count Differentiation & XX \\
Temporal & Temporal Flow Variability Index & XX \\
\hline
Spatial & Bird-Eye View Awareness & XX \\
Spatial & Heat Map Visualization & XX \\
Spatial & Space Utilization Score & XX \\
Spatial & Object Interaction Zones & XX \\
Spatial & Incident Proximity Mapping & XX \\
\hline
Spatiotemporal & Movement Pattern Detection & XX \\
Spatiotemporal & Bottleneck Identification & XX \\
Spatiotemporal & Directional Flow Estimation & XX \\
Spatiotemporal & Queue Formation Detection & XX \\
Spatiotemporal & Crowd Density Forecasting & XX \\
Spatiotemporal & Event Surge Prediction & XX \\
\hline
Safety-Oriented & Emergency Route Clearance Indicator & XX \\
Safety-Oriented & Anomaly Detection & XX \\
Safety-Oriented & VIP Flow Protection Zones & XX \\
\hline
Retail-Oriented & Shopfront Engagement Time & XX \\
Retail-Oriented & Retail Conversion Flow Ratio & XX \\
\hline
\end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{}
    \caption{Caption}
    \label{fig:placeholder}
\end{figure}


==> table_1.tex <==
\begin{table*}[t]
\centering
\caption{Reframing UX Metrics from Pre-AI Systems to Post-AI Human- and Society-in-the-Loop Design}
\label{tab:ux_metrics_hitl}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|p{2.5cm}|p{3cm}|p{3cm}|p{3.5cm}|p{4cm}|}
\hline
\textbf{UX Dimension} & \textbf{Pre-AI UX Focus} & \textbf{Pre-AI Metrics} & \textbf{Post-AI UX Focus (HITL)} & \textbf{New UX Metrics (Interview-Derived)} \\
\hline
Decision Making & Task execution & Task success rate & Sensemaking and judgment & Decision confidence score \\
\hline
Control & Full automation & Automation rate & Shared human–AI control & Perceived controllability \\
\hline
Trust & System reliability & FPR / FNR & Trust calibration & Trust calibration index \\
\hline
Transparency & Output visibility & Explainability logs & Interpretability & Explanation usefulness rating \\
\hline
Responsiveness & Speed & Latency & Early situational awareness & Early-warning usefulness \\
\hline
Cognitive Load & Efficiency & Task time & Cognitive support & Cognitive load balance score \\
\hline
Situational Awareness & Static monitoring & Camera uptime & Contextual pattern awareness & Situational clarity score \\
\hline
Safety Oversight & Rule-based alerts & Alert count & Context-aware risk sensing & False alarm tolerance \\
\hline
Adaptability & Fixed thresholds & Threshold accuracy & Contextual customization & Customization satisfaction \\
\hline
Accountability & System-centric logs & Log completeness & Shared responsibility & Accountability clarity index \\
\hline
Learning and Feedback & Offline retraining & Update cycles & Continuous feedback loop & Feedback usefulness score \\
\hline
Social Acceptance & Not considered & N/A & Societal trust and legitimacy & Perceived intrusiveness \\
\hline
\end{tabular}
\end{table*}


This table contrasts traditional pre-AI usability-oriented metrics with post-AI UX metrics derived from stakeholder interviews and focus groups. The proposed metrics emphasize human judgment, trust calibration, accountability, and societal acceptance, aligning with Human- and Society-in-the-Loop design principles.
